Composing Diverse Policies for Temporally Extended Tasks

Robot control policies for temporally extended and sequenced tasks are often characterized by discontinuous switches between different local dynamics. These change-points are often exploited in hierarchical motion planning to build approximate models and to facilitate the design of local, region-specific controllers. However, it becomes combinatorially challenging to implement such a pipeline for complex temporally extended tasks, especially when the sub-controllers work on different information streams, time scales and action spaces. In this paper, we introduce a method that can compose diverse policies comprising motion planning trajectories, dynamic motion primitives and neural network controllers. We introduce a global goal scoring estimator that uses local, per-motion primitive dynamics models and corresponding activation state-space sets to sequence diverse policies in a locally optimal fashion. We use expert demonstrations to convert what is typically viewed as a gradient-based learning process into a planning process without explicitly specifying pre- and post-conditions. We first illustrate the proposed framework using an MDP benchmark to showcase robustness to action and model dynamics mismatch, and then with a particularly complex physical gear assembly task, solved on a PR2 robot. We show that the proposed approach successfully discovers the optimal sequence of controllers and solves both tasks efficiently.

==> content/9-supplementary_material.tex <==
\section*{Supplementary Material}

This material includes additional detail around the controller components used for experimentation. For obtaining the neural policies (e.g. Figure.\ref{fig:gear_peg}) we used the following rule of thumb:

\begin{itemize}
    \item We use a Behaviour Cloning loss with the VAE loss to train our policy models with Adam with $\alpha = 0.001$ with weight decay of $1e^{-6}$. We obtained 50 demonstrations of each subtask.

    \item Our input image has a size of $128x128$ pixels. We observe that the Neural Network Policy does not require a sophisticated feature extractor like ResNet50, ResNet101 to create necessary features for the task. Using those extractors leads to the same final performance, but increases the training time significantly. We use 5 convolutional layers of 4x4 filters with batch normalization and leaky ReLUs.

    \begin{table}[h]
        \centering
        \begin{tabular}{lcc}
        \hline
                   & Sub Task Performance & Full Task Performance \\ \hline
        ResNet50   & 10/10                & 10/10                 \\
        ResNet101  & 10/10                & 10/10                 \\
        Small Conv & 10/10                & 10/10                
        \end{tabular}
    \end{table}
    
    \item Additional ``what-if'' \textit{(it's tilted, flipped, not visible, etc.)} training examples were detrimental to the performance of the model. In order to incorporate that part of the state space, a full set of overlapping and interpolating examples need to be provided.
\end{itemize}

\begin{figure*}
\centering
\includegraphics[width=1.\linewidth]{images/123h.eps}
\caption{The execution of a neural network policy for inserting the gear on the peg. }
\label{fig:gear_peg}
\end{figure*}


